OmniOPD: Logit-Free On-Policy Distillation via Speculative Verification

On-Policy Distillation (OPD) trains a student model on its own generative trajectories under dense token-level feedback from a stronger teacher, mitigating both the off-policy distribution shift of Supervised Fine-Tuning (SFT) and the sparse credit assignment of Reinforcement Learning (RL). However, standard OPD faces two coupled limitations. First, it requires direct access to the teacher's token-level logits, excluding a broad class of capable proprietary models from serving as teachers. Second, the token-level logit signal itself is brittle, depending on a narrow overlap of plausible next tokens between teacher and student, and prone to amplifying degenerate patterns such as repetition loops. In this paper, we introduce OmniOPD, a novel framework that addresses both limitations through a logit-free, chunk-level supervision signal. OmniOPD replaces deterministic logit matching with Monte Carlo rollouts that approximate the teacher's local preferences through a continuous semantic similarity metric over multi-token chunks, and concentrates this supervision via a peak-entropy scheduler that audits the student only at its high-uncertainty reasoning forks. A Dirichlet-Multinomial Bayesian prior and a base-model KL anchor further bound the variance of discrete sampling and prevent policy collapse across unaudited tokens. Across competitive benchmarks, OmniOPD surpasses the standard OPD approach by up to +28.64% on math, confirming that chunk-level semantic verification extracts a more reliable learning signal than token-level logit matching, whose high information density is offset by significant noise and brittleness. Furthermore, when paired with stronger black-box teachers such as Claude-4.5-Haiku and Gemini-2.5-Flash, OmniOPD achieves an additional +9.54% relative on math over its open-weight teacher counterpart, advancing the student past the performance of self-exploratory RL.

==> sections/0_abstract.tex <==
On-Policy Distillation (OPD) trains a student model on its own generative trajectories under dense token-level feedback from a stronger teacher, mitigating both the off-policy distribution shift of Supervised Fine-Tuning (SFT) and the sparse credit assignment of outcome-based Reinforcement Learning (RL).
%
However, standard OPD faces two coupled limitations. 
%
First, it requires direct access to the teacher's token-level logits, excluding a broad class of capable proprietary models. 
%
Second, the token-level logit signal itself is brittle, depending on a narrow overlap of plausible next tokens between teacher and student, and prone to amplifying degenerate patterns such as repetition loops.
%
We introduce \textbf{\ours}, a novel framework that addresses both limitations through a logit-free, chunk-level supervision signal.
%
\ours replaces deterministic logit matching with Monte Carlo rollouts that approximate the teacher's preferences through a continuous semantic similarity metric over multi-token chunks, and concentrates this supervision via a peak-entropy scheduler that audits the student only at its high-uncertainty reasoning forks.
%
Across mathematical reasoning and competitive programming benchmarks, \ours outperforms SFT by up to +45.31\% relative on math and surpasses standard OPD approach by up to +28.64\% on mathematical reasoning, confirming that chunk-level semantic verification extracts a cleaner and more reliable learning signal than token-level logit matching.

==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:introduction}

On-Policy Distillation (OPD) has emerged as a central paradigm for post-training open-weight reasoning models~\citep{agarwal2024policy, lu2025onpolicydistillation, song2026survey}.
%
By having the student generate its own reasoning trajectories and querying a stronger teacher to score them, OPD combines the dense token-level supervision of Supervised Fine-Tuning (SFT) with the on-policy exploration of Reinforcement Learning (RL), mitigating both the distribution shift of imitating offline demonstrations~\citep{huan2025does} and the sparse credit assignment of outcome-based RL methods such as GRPO~\citep{shao2024deepseekmath, chen2025exploration}.
%

Despite these strengths, standard OPD inherits two coupled limitations that both stem from using the teacher's token-level log-probabilities as the supervision signal.
%
First, standard OPD approaches~\citep{agarwal2024policy, lu2025onpolicydistillation} requires direct read-out of the teacher's exact next-token logits. 
%
This limitation is increasingly restrictive, as a broad class of capable proprietary models, such as Claude~\citep{anthropic2025system}, and the wider commercial LLM ecosystem~\citep{aubakirova2026state}, return only text, not logits, and are therefore excluded from the OPD pipeline entirely~\citep{song2026survey}.

%
Second, even when full logit access is available, token-level matching is a surprisingly brittle target. 
%
Recent studies of OPD failure modes~\citep{li2026rethinking, luo2026demystifying, fu2026revisiting} show that the effective supervision signal lives in the narrow overlap between the teacher's and student's plausible next-token sets --- a small set of plausible next tokens that concentrates the bulk of the gradient mass.
%
This narrow region is fragile: it degrades when teacher and student reason in stylistically different ways, becomes uninformative or actively harmful on degenerate prefixes such as repetition loops, and is further disrupted by tokenizer mismatches between proprietary and open-weight model families~\citep{fu2026revisiting}.
%
The high-dimensional logit distribution offers far less reliable supervision than its information density would suggest.
%
% }
% The alignment and enhancement of Large Language Models (LLMs) currently rely on two dominant fine-tuning paradigms: Supervised Fine-Tuning (SFT) and Reinforcement Learning (RL)~\citep{openai2023gpt4, yang2025qwen3}.
%
% SFT provides dense, token-level supervision, but operates strictly off-policy. 
%
% By forcing the student to mimic offline demonstrations, SFT exposes the model to severe distribution shifts during inference~\citep{huan2025does}.
%
% Conversely, RL methods such as Group Relative Policy Optimization (GRPO) address this by training on-policy, allowing the model to learn from its own actively generated trajectories. 
%
% However, RL is bottlenecked by sparse, outcome-based rewards, making granular credit assignment exceedingly difficult for complex, multi-step reasoning tasks~\citep{chen2025exploration}.
%
% On-Policy Distillation (OPD) elegantly resolves this dichotomy. 
%
% By querying a superior teacher model to evaluate the student's active generations, OPD combines the robustness of on-policy exploration with the dense, step-by-step supervision of SFT~\citep{lu2025onpolicydistillation, agarwal2024policy}. 
%
% Yet, the standard formulation of OPD is fundamentally constrained by a critical architectural barrier: it requires white-box access to the teacher's exact token-level logits to compute the distillation loss. 
%
% This creates a severe limitation for the open-source community, as the most advanced reasoning frontier models are black-boxes.
% \zz{I am thinking in general we don't need to make the statement that the best models are black-box (even if they do), we can just say black-box models are also a broad class of models that could've been great teachers. Another thing I am thinking is that, since our performance does beat standard OPD, we can also claim that chunk-level semantic verification extracts a richer learning signal than token-level logit matching? So the new framing could be that the motivation is 1. removes the need to access logit; 2. we provide a better dense signal than token logit. I edited the abstract to reflect this, but what do you think?}
% \yf{I think chunk-level verification makes OPD feasible for black-box models with no logits or shared tokenizer, but saying it provides richer information than token-level logits does not seem accurate to me.}
%
This motivates our central question: Can dense on-policy distillation be performed without access to the teacher's logits, and what alternative dense supervision signal could match, or surpass, logit-based matching?
%

We answer both questions with \textbf{\ours}, a logit-free framework that supervises the student through a multi-token, semantic-level signal estimated from text alone.
%
Our approach builds on \textit{Monte Carlo estimation}~\citep{kroese2014monte}. 
%
Rather than requiring deterministic logit distributions, \ours approximates the teacher's local preferences by sampling multiple discrete rollouts and estimating the teacher's \textit{true} probability density from their semantic similarity to the student's generation. 
%
To make this computationally viable under restricted query budgets, we propose a peak-entropy \textit{chunk scheduling}. 
%
Instead of querying the teacher at every token, \ours selectively audits chunk of student tokens at the high-uncertainty decision boundaries in the student's reasoning trajectory, which is the point where corrective supervision is most valuable.
%
Finally, to counteract the high variance and zero-probability traps inherent in discrete sampling, we introduce a \textit{Bayesian smoothing step}~\citep{robbins1992empirical}. 
%
By anchoring the empirical Monte Carlo estimates with the student's base-model prior, \ours extracts a variance-reduced gradient signal, while a separate base-model KL anchor on un-audited tokens prevents policy collapse across the trajectory's unsupervised gaps.
%

Across mathematical reasoning and competitive programming benchmarks, \ours substantially outperforms SFT and, more strikingly, frequently outperforms white-box OPD~\citep{lu2025onpolicydistillation} even when full teacher logits are available. 
%
This finding provides empirical support for our second motivation, where a coarser but cleaner signal yields stronger gradients than the high-bandwidth but noisy token-level distribution that white-box OPD optimizes.
%
When paired with stronger black-box teachers such as Claude-4.5-haiku~\citep{anthropic2025system} and Gemini-2.5-flash~\citep{comanici2025gemini}, \ours further advances the student past the performance ceiling of self-exploratory GRPO~\citep{shao2024deepseekmath} on the same model. 
%
% Extensive evaluations across complex mathematical reasoning and competitive programming benchmarks validate the efficacy of our framework. 
%
% \ours achieves substantial performance gains over standard SFT across various open-weight and closed-source teacher setups, delivering up to +7.40\% gain over offline SFT on mathematical reasoning with Claude-4.5-haiku as the teacher. 
%
% Remarkably, \ours frequently surpasses full-logit white-box OPD by granting the student localized semantic flexibility rather than enforcing strict token-by-token imitation. 
%
% Furthermore, when leveraging frontier models such as Claude and Gemini as teachers, \ours decisively breaks the performance ceilings of standard GRPO empowering smaller student models to achieve extraordinary reasoning capabilities.
%
In summary, our main contributions are as follows:
\begin{itemize}[leftmargin=*, nosep]
    % \item We formalize the problem of black-box on-policy distillation and introduce \ours, a framework that successfully bypasses the white-box logit bottleneck via semantic Monte Carlo estimation.
    \item We propose \ours, a logit-free, chunk-level OPD framework that addresses both the white-box access requirement of standard OPD and the brittleness of its token-level supervision signal.
    %
    % \item We design an efficient peak-entropy scheduling mechanism that concentrates teacher verification at the trajectory's most uncertain reasoning forks, coupled with a Bayesian smoothing mechanism and trust-region penalty to mathematically stabilize discrete sampled targets and prevent catastrophic policy collapse.
    \item We introduce three components that make \ours tractable and stable: a peak-entropy scheduler that concentrates teacher verification at the trajectory's most uncertain reasoning forks, a Dirichlet-Multinomial Bayesian prior that stabilizes the discrete Monte Carlo estimates, and a trust-region KL penalty that prevents policy collapse across un-audited tokens. 
    %
    We provide formal guarantees on estimation error, gradient variance, and trajectory stability.
    %
    \item We demonstrate empirically that \ours outperforms SFT by up to +45.31\% relative on mathematical reasoning and +18.52\% on competitive programming, exceeds white-box OPD by up to +28.64\% on mathematical reasoning, and, when paired with stronger black-box teachers such as Claude-4.5-haiku and Gemini-2.5-flash, advances the student past the performance ceiling of self-exploratory GRPO.
    % \item We demonstrate empirically that \ours consistently outperforms SFT, matches or exceeds white-box OPD (e.g., +4.92\% on average in mathematical reasoning), and seamlessly scales to frontier commercial systems to surpass standard RL limits.
\end{itemize}

==> sections/2_related.tex <==
\section{Related Work}
\label{sec:related_work}

\paragraph{Offline policy distillation of LLMs.}
The traditional paradigm for transferring complex reasoning capabilities from frontier models to smaller, more deployable models is offline knowledge distillation~\citep{hsieh2023distilling, shridhar2023distilling, kim2016sequence}. 
%
Early approaches primarily relied on sequence-level distillation from black-box APIs, querying more capable models to generate high-quality Chain-of-Thought (CoT)~\citep{wei2022chain} trajectories and training the student model to mimic these sequences via SFT~\citep{ho2022large, zhou2024teaching, lee2024mentor}. 
%
While effective for basic instruction following, this sequence-level imitation often fails to capture the nuanced, token-by-token reasoning dynamics of the teacher.
%
% \zz{
With the emergence of highly capable open-source models~\citep{grattafiori2024llama, abdin2024phi, yang2025qwen3, guo2025deepseek, kamath2025gemma, team2025kimi, xiao2026mimo}, the field increasingly shifted toward more fine-grained, white-box distillation techniques that directly optimize the student against the teacher's continuous output distributions via Forward Kullback-Leibler (KL) divergence or token-level logit matching~\citep{gu2024minillm, wen2023f}.
% }
%
However, whether utilizing black-box textual trajectories or white-box logits, these approaches are fundamentally off-policy: the student is trained on the teacher's static state distribution, leading to inevitable distribution shift and exposure bias during deployment.
%


\paragraph{On-policy distillation and its limitations.}
To mitigate the exposure bias inherent to offline methods, OPD shifts the learning objective to the student's own generated distribution~\citep{agarwal2024policy, lu2025onpolicydistillation}. 
%
In standard OPD frameworks, the student model actively generates reasoning trajectories that are then evaluated and scored by the teacher model, bridging the gap between training and inference distributions. 
%
Recent variants have expanded this paradigm to self-OPD, where a model iteratively improves through its own on-policy feedback~\citep{zhao2026self, he2026self, hubotter2026reinforcement}, as well as generalized OPD frameworks designed to handle architectural differences such as mismatched tokenizers between the student and teacher model~\citep{patino2025_unlocking}.
%
% \zz{
Despite these advancements, recent analyses have revealed that the token-level logit signal underlying standard OPD is surprisingly brittle. 
%
\citet{li2026rethinking} show that the effective supervision signal concentrates in the narrow overlap between teacher and student plausible next-token sets, and that a teacher with strong benchmark accuracy can fail to improve a student whose reasoning trajectories fall outside this overlap. 
%
\citet{luo2026demystifying} document a systematic collapse mode in which degenerate prefixes such as repetition loops accidentally receive large positive gradient signal, since locally predictable tokens are assigned high probability by the teacher. 
%
\citet{fu2026revisiting} further show that single-sampled-token feedback is statistically noisy, and that tokenizer mismatches between teacher and student introduce a class of spurious disagreements that no amount of logit access can resolve. 
%
These findings establish token-level logit matching as a structurally fragile supervision signal, motivating the chunk-level semantic approach we develop in this paper.
%
Beyond brittleness, standard OPD also faces a structural access barrier that computing the Reverse KL divergence between student and teacher requires explicit access to the teacher's token probabilities~\citep{yang2026learning}. 
%
Consequently, OPD with proprietary teachers has remained largely unexplored. 
%
\citet{ye2025black} recently introduced Generative Adversarial Distillation (GAD), which trains an auxiliary discriminator as an evolving reward model in a minimax game with the student.
%
While GAD bypasses the logit requirement, its discriminator yields only a sequence-level scalar score, providing coarser feedback than the per-step supervision of standard OPD, and requiring an additional model to train and maintain. 
%
\ours instead recovers dense, chunk-level supervision directly from teacher rollouts through Monte Carlo semantic estimation, without any auxiliary network, and matches or exceeds white-box logit matching when full teacher access is available.
%
% }

% Despite these advancements, standard OPD fundamentally relies on white-box teachers, as computing the Reverse KL divergence requires explicit access to the teacher's token probabilities \citep{yang2026learning}. Consequently, OPD with frontier black-box models has remained largely unexplored. While \citet{ye2025black} explores online distillation from black-box models via adversarial methods, such approaches necessitate training an auxiliary reward model and only yield sparse scalar feedback, lacking the dense optimization signals characteristic of standard OPD. 

% \ours is the first framework to bridge the gap between rigorous OPD and black-box distillation without relying on adversarial mechanisms. By mathematically estimating the token probabilities via Bayesian-smoothed Monte Carlo rollouts, our method introduces a stable, probabilistically grounded pathway to distill the active reasoning capabilities of frontier black-box models.

==> sections/3_method.tex <==
\section{Methodology}
\label{sec:workflow}

\subsection{Preliminaries}
\paragraph{Offline Supervised Fine-Tuning (SFT).}
The standard paradigm for transferring reasoning capabilities from a strong teacher model to a smaller student model is SFT. 
%
Given a dataset of instructions $x$ and corresponding reasoning trajectories $y = (y_1, y_2, \dots, y_T)$ generated by a teacher, SFT optimizes the student policy $\pi_\theta$ via maximum likelihood estimation. 
%
The objective minimizes the standard cross-entropy loss:
\begin{equation}
    \mathcal{L}_{\text{SFT}}(\theta) = - \mathbb{E}_{(x, y) \sim \mathcal{D}} \left[ \sum_{t=1}^{T} \log \pi_\theta(y_t \mid x, y_{<t}) \right]
\end{equation}
%
While efficient, offline SFT inherently suffers from exposure bias and distribution shift, as the student is trained on the teacher's static state distribution, not its own~\citep{lu2025onpolicydistillation}.
%


\paragraph{Online On-Policy Distillation (OPD).}
% To mitigate the distribution shift of SFT, OPD shifts the learning paradigm from imitation to active exploration. 
% \zz{
OPD addresses this exposure bias by training on the student's own generations rather than the teacher's static trajectories.
%
Let $\hat{y} \sim \pi_\theta(\cdot \mid x)$ be a trajectory sampled from the student policy.
%
Standard OPD minimizes a per-token divergence (most commonly the Reverse KL divergence) between the student and the true teacher policy $\pi_{teacher}^*$~\citep{agarwal2024policy, lu2025onpolicydistillation}:
%
% }
%
% In OPD, the student model generates its own reasoning trajectory $\hat{y} \sim \pi_\theta(\cdot \mid x)$ (i.e., operating on-policy). 
%
% The teacher model then verifies this student-generated trajectory to provide a learning signal. 
%
% Using our established notation, standard OPD minimizes a divergence—typically the Reverse KL divergence between the student's policy $\pi_\theta$ and the true, exact teacher policy $\pi_{teacher}^*$:
\begin{equation}
\resizebox{\columnwidth}{!}{$\displaystyle
    \mathcal{L}_{\text{OPD}}(\theta) = \mathbb{E}_{x \sim \mathcal{D}, \hat{y} \sim \pi_\theta} \!\left[ \sum_{t=1}^{|\hat{y}|} D_{\text{KL}} \Big( \pi_\theta(\cdot \mid x, \hat{y}_{<t}) \parallel \pi_{\text{teacher}}^*(\cdot \mid x, \hat{y}_{<t}) \Big) \right]
$}
\label{eq:opd_loss}
\end{equation}
%
By exploring its own action space and receiving corrective feedback from the teacher distribution $\pi_{teacher}^*$, the student learns a more robust policy that bridges the gap between training and inference distributions.
%

% \paragraph{The White-Box Bottleneck.}
% A critical limitation of current OPD methodologies is their strict reliance on \textit{white-box} teacher models. 
% %
% To compute the exact KL divergence for optimization, the objective requires direct access to the teacher's continuous token-level log-probabilities, $\log \pi_{teacher}^*(y_t \mid x, y_{<t})$. 
% %
% Consequently, standard OPD frameworks cannot utilize frontier black-box models as teachers because these black-box systems do not output the required token-level logits.

\subsection{\ours}
% \zz{WIP}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figure/omniopd_diagram.png}
    \caption{Overview of \ours. \textbf{Entropy-Driven Chunk Selection:} Given an input prompt $x$, the student model generates an on-policy trajectory. \ours first identifies critical reasoning forks by locating local peaks in predictive entropy. \textbf{Chunk-level Teacher Critic:} For each selected chunk, the trajectory prefix $y_{<c}$ is passed to the teacher. The teacher generates multiple Monte Carlo rollouts, which are then evaluated against the student's generated chunk via a continuous semantic similarity metric. \textbf{Calculate Loss and Update Student:} The student policy is updated by applying the distillation loss exclusively to the audited tokens. Simultaneously, a Reference KL anchor is applied across the unaudited tokens to constrain the policy shift.}
    \label{fig:omniopd_framework}
\end{figure*}

% To bypass the white-box bottleneck, a natural approach is to approximate the true teacher policy $\pi_{teacher}^*$ using only the discrete textual outputs via a Monte Carlo (MC) method. 
%
% At every generation step $t$, one could theoretically prompt the teacher to generate multiple independent rollouts and calculate the empirical frequency of the student's exact next token. 
%
% However, executing this naive token-by-token estimation across an entire reasoning trajectory of length $T$ is economically intractable due to the massive volume of teacher queries required. 
%
% Furthermore, it is statistically brittle; vocabulary and tokenization mismatches between distinct models make exact token-level matches highly improbable, yielding sparse, zero-reward gradients. 
%
% \zz{
\ours addresses both limitations of standard OPD identified in \secref{sec:introduction} through replacing the token-level logit signal with a chunk-level semantic signal estimated from text along.
%
As illustrated in \figref{fig:omniopd_framework}, \ours has three components: a peak-entropy scheduler that selects high-uncertainty chunks from the student's trajectory (\secref{subsubsec:chunk_selection}), a chunk-level teacher critic that estimates the teacher's preference through Monte Carlo rollouts evaluated by semantic similarity (\secref{subsubsec:speculative_verification} and~\ref{subsubsec:bayesian_smoothing}), and a trust-region anchor that prevents policy drift on un-audited tokens (\secref{subsubsec:trust_region}).
%
The full algorithm is presented in Algorithm~\ref{alg:OPD} in \appref{app:supp_omniopd}.
%
% }
% To resolve these dual bottlenecks, as illustrated in Figure \ref{fig:omniopd_framework}, \ours introduces a progressive, chunk-level formulation bounded by Bayesian priors and trust regions. The full algorithm is presented in Algorithm \ref{alg:OPD} in Appendix.


\subsubsection{Chunk-Level Distillation via Speculative Verification}
\label{subsubsec:speculative_verification}
% \zz{
Our logit-free distillation is built on Monte Carlo estimation of the teacher's preference.
%
A naive token-level instantiation --- querying the teacher at every step $t$ and estimating the empirical frequency of the student's exact next token --- is infeasible because the per-token query volume scales as $O(T)$ over reasoning trajectories of length $T$.
%
Tokenization differences between distinct model families may also cause the student's exact next token to not appear in any teacher rollout, producing sparse, zero-gradient updates that destabilize optimization.
%
To resolve these issues, \ours instead groups consecutive tokens into chunks of $C$ tokens and applies a single teacher query per chunk, reducing the query volume by a factor of $O(T/C)$ and shifting the matching signal from exact tokens to semantic similarity.
%
% }
% To resolve the severe query overhead of token-level queries, we fundamentally restructure the temporal resolution of distillation. 
%
% Instead of prompting the teacher at every generation step to evaluate individual student tokens, we apply the teacher-critic such that a single teacher query evaluates a contiguous chunk of $C$ tokens, drastically reducing the query volume by a factor of $\mathcal{O}(T/C)$.
%
This chunk-level paradigm is structurally inspired by the verification phase of Speculative Decoding~\citep{leviathan2023fast,chen2023accelerating}, where a large target model parallel-verifies a sequence drafted by a smaller model. 
%
In our framework, we treat each $C$-token block as a single, cohesive verification unit.
%

Let the student model generate an on-policy reasoning trajectory $y \sim \pi_\theta(\cdot \mid x)$. 
%
From this trajectory, we select $M$ non-overlapping chunks of length $C$ (the selection mechanism is later detailed in \secref{subsubsec:chunk_selection}).
%
For a student chunk $c$, the black-box teacher receives the historical prefix $y_{<c}$ and generates $N$ independent Monte Carlo rollouts $\{y_{\text{teacher}}^{(i)}\}_{i=1}^N$. 
%
Notably, as frontier teacher models and local student models rarely share the same tokenizer, even at chunk level, computing exact probability matches between teacher rollouts and the student's chunk remains infeasible.
% strict token-level probability matching is structurally impossible.
%
To resolve this tokenizer mismatch, \ours evaluates the student's chunk against the teacher rollouts using a continuous semantic similarity function $\phi : (y_c, y_{\text{teacher}}) \mapsto [0, 1]$
% $\phi \in [0, 1]$ 
(e.g., ROUGE-1 unigram overlap~\citep{lin-2004-rouge}). 
%
The aggregate semantic similarity $k_{\text{sem}}^{(c)}$ for chunk $c$ is then computed as:
\begin{equation}
    k_{\text{sem}}^{(c)} = \sum_{i=1}^{N} \phi(y_c, y_{\text{teacher}}^{(i)})
    \label{eq:aggregate_semantic_similarity}
\end{equation}
%
By shifting the measurement from tokens to semantics over a continuous $C$-token window, we effectively verify the student's conceptual milestones across distinct model architectures without penalizing stylistic deviations or vocabulary mismatches.
%


\subsubsection{Bayesian Smoothing for Sparse Signals}
\label{subsubsec:bayesian_smoothing}
While the chunk-level formulation reduces the query overhead, estimating the teacher policy from a limited sampling budget $N$ introduces high variance. 
%
A naive frequentist estimation $\hat{\pi}_{\text{freq}}^{(c)} = k_{\text{sem}}^{(c)}/N$ risks gradient explosion during optimization: when the teacher's sparse rollouts yield zero semantic matches, the log-loss is driven to infinity. 

To stabilize this estimation, we model the teacher's feedback using a Dirichlet-Multinomial conjugate prior. 
%
% We first compute the student's normalized probability over the chunk to serve as a structural base prior:
Taking the student's own per-chunk normalized probability as the prior:
%
\begin{equation}
    \bar{\pi}_\theta^{(c)} = \left( \prod_{t \in c} \pi_\theta(y_t \mid x, y_{<t}) \right)^{\frac{1}{C}}
    \label{eq:student_prior}
\end{equation}
%
The stabilized Bayesian target proxy $\hat{\pi}_{\text{teacher}}^{(c)}$, parameterized by prior strength $\alpha$ is then:
%
\begin{equation}
    \hat{\pi}_{\text{teacher}}^{(c)} = \frac{k_{\text{sem}}^{(c)} + \alpha \cdot \bar{\pi}_\theta^{(c)}}{N + \alpha}
\label{eq:bayesian_smooth_estimation}
\end{equation}
%
% Theorem~\ref{theorem:bayesian_bound} (\secref{sec:theoretical_analysis}) shows that this formulation strictly bounds the Mean Squared Error (MSE) of the proxy $\hat{\pi}_{\text{teacher}}^{(c)}$ and guarantees finite, stable gradients even under complete teacher disagreement ($k_{\text{sem}}^{(c)} = 0$), preventing catastrophic divergence during on-policy updates.
Theorem~\ref{thm:gradient_stability} demonstrates that this Bayesian proxy not only strictly bounds the Mean Squared Error (MSE) of $\hat{\pi}_{\text{teacher}}^{(c)}$, but also acts as a mathematical failsafe. By anchoring to the student's prior, it guarantees bounded, non-zero gradients even when teacher rollouts yield zero semantic matches ($k_{\text{sem}}^{(c)} = 0$), completely eliminating the risk of supervision collapse during training.


\subsubsection{Entropy-Driven Chunk Selection
}
\label{subsubsec:chunk_selection}
Under a budget of $M$ chunks per trajectory, the method by which we select these windows determines distillation efficiency. 
%
Reasoning trajectories oftentimes contain long segments of low-complexity transitions (e.g., formatting and deterministic arithmetic), where teacher verification provides negligible gradient signal. 
%
% Allocating our limited evaluations to these low-complexity segments wastes distillation bandwidth and provides a negligible gradient signal.
%
To maximize the marginal utility of each critic, we aim to target teacher verification at at the high-uncertainty reasoning forks where the student's policy diverges. 
%

As the student model $\pi_\theta$ is fully accessible, we use its internal predictive entropy as a proxy for this local uncertainty.
%
At each generation step $t$, we compute the entropy of the student's output vocabulary distribution:
%
\begin{equation}
    \mathcal{H}_t = - \sum_{v \in \mathcal{V}} \pi_\theta(v \mid x, y_{<t}) \log \pi_\theta(v \mid x, y_{<t})
\end{equation}
%
where $\mathcal{V}$ is the vocabulary space. 
%
A low entropy $\mathcal{H}_t$ indicates a deterministic transition; while high entropy indicates a complex decision boundary.
%

To capture these decision boundaries, we select a set $\mathcal{A}$, which consists of the $M$ tokens with the highest entropy from the trajectory, for chunk formation:
% employ a peak-anchored selection strategy, where we sort the trajectory to identify the set of $M$ anchor tokens, $A$, that exhibit the highest absolute entropy:
\begin{equation}
    \mathcal{A} = \mathop{\arg\max}\limits_{t \subset \{1 \dots T\}, |\mathcal{A}|=M} (\mathcal{H}_t)
\end{equation}
%
For each anchor token $t^* \in \mathcal{A}$, we extract a contiguous $C$-token chunk that encompasses this point of divergence as the audited chunk.
%
To maintain structural integrity, any dynamically formed chunks that overlap are merged or resampled.
%
By anchoring the $M$ chunks to the highest-entropy positions in the trajectory, this selection mechanism ensures that the Bayesian proxy targets ($\hat{\pi}_{\text{teacher}}^{(c)}$) are applied where the student's policy is most uncertain and requires the most correction.
%


\subsubsection{Trust Region Anchoring}
\label{subsubsec:trust_region}
While our peak-entropy selection places the $M$ audited chunks at the most informative positions, it leaves the remaining $|\mathcal{U}| = T - M \cdot C$ tokens un-audited. 
%
% Let $U$ denote this set of un-audited tokens, where $|\mathcal{U}| = T - M \cdot C$. 
%
Optimizing a policy on these sparse, localized signals risks policy degeneration, as the student model $\pi_\theta$ might exploit structural shortcuts, generate incoherent text between audited chunks, or collapse its entropy to artificially shorten the trajectory length.
%

For all un-audited tokens $t \in \mathcal{U}$, we apply a KL divergence penalty against the reference policy $\pi_{\text{ref}}$, which is the frozen copy of the student's initial weights. 
%
By Pinsker's inequality~\citep{pinsker1964information}, minimizing $D_{KL}(\pi_{\text{ref}} \parallel \pi_\theta)$ bounds the Total Variation shift of the student's policy, acting as a trust region that constrains drift in the unsupervised regions (formalized in \theoremref{theorem:trust_region}).
%
Consequently, policy updates concentrate on the audited chunks while the trust region holds the un-audited tokens close to $\pi_{\text{ref}}$.
%
% Minimizing the divergence $D_{KL}(\pi_{ref} \parallel \pi_\theta)$ effectively bounds the Total Variation shift of the student's policy. 
%
% This elastic penalty acts as a robust trust region, forcing the student to maintain its foundational fluency and verbose reasoning structure across the unsupervised gaps.
%
% Consequently, the model only allows significant policy updates exactly where the Bayesian teacher explicitly provides corrective gradients.
%


\paragraph{The \ours optimization objective.}
% The final \ours framework seamlessly unifies the Bayesian-smoothed chunk distillation with the token-level trust region penalty. 
Combining chunk-level Bayesian distillation with the token-level trust region, the complete \ours objective is:
\begin{equation}
\resizebox{\columnwidth}{!}{$\displaystyle
\begin{split}
    \mathcal{L}_{\ours}(\theta) &= \underbrace{-\mathbb{E}_{\hat{y} \sim \pi_\theta} \!\Bigg[ \sum_{c=1}^{M} \hat{\pi}^{(c)}_{\text{teacher}} \sum_{t \in c} \log \pi_\theta(y_t \mid x, y_{<t}) \Bigg]}_{\mathcal{L}_{\text{chunk}}(\theta)} \\
    &\quad + \underbrace{\beta \sum_{t \in \mathcal{U}} D_{\text{KL}}\bigl(\pi_{\text{ref}}(\cdot \mid x, y_{<t}) \,\|\, \pi_\theta(\cdot \mid x, y_{<t})\bigr)}_{\text{trust-region anchor}}.
\end{split}
$}
\label{eq:omniopd_loss}
\end{equation}
where $\beta$ controls the strength of the trust-region anchor.
%
By minimizing $\mathcal{L}_{\ours}$, the student model systematically aligns its critical, high-entropy reasoning junctions with the frontier black-box teacher, while the trust-region penalty ensures the global stability and coherence of the resulting long-horizon trajectory.
%
A comprehensive theoretical analysis is provided in Appendix \ref{sec:theoretical_analysis}, where we formally demonstrate how these core mechanisms mathematically eliminate gradient instability, guarantee rollout sufficiency under tight budgets, and strictly bound the distributional drift of un-audited tokens.



==> sections/4_theory.tex <==
\section{Theoretical Analysis of \ours}
\label{sec:theoretical_analysis}
% \zz{
In this section, we provide a theoretical analysis of \ours's three core design components --- chunk-level loss formulation (\eqnref{eq:omniopd_loss}), Bayesian-smoothed estimation (\eqnref{eq:bayesian_smooth_estimation}), and trust-region anchoring on un-audited tokens --- by tying each one to a specific failure mode it prevents.
%
\paragraph{Setup.}
We assume the semantic similarity function $\phi$ (as in \eqnref{eq:aggregate_semantic_similarity}) takes values in $[0,1]$, teacher rollouts $\{y^{(i)}_{\text{teacher}}\}_{i=1}^N$ are i.i.d.\ samples from $\pi^*_{\text{teacher}}(\cdot \mid x, y_{<c})$, the student prior $\bar{\pi}^{(c)}_\theta > 0$ (as in \eqnref{eq:student_prior}) as a geometric mean of strictly positive per-token probabilities, and the score function $\nabla_\theta \log \pi_\theta(y_t \mid \cdot)$ is bounded, which is a standard assumption for softmax-output transformer policies. 
%
For each chunk $c$, we define the true expected similarity as
%
\begin{equation}
    \mu_c := \mathbb{E}_{y' \sim \pi^*_{\text{teacher}}(\cdot \mid x, y_{<c})}\!\left[\phi(y_c, y')\right] \in [0,1].
    \label{eq:mu_c_def}
\end{equation}
%
The empirical frequentist estimator $\hat{\pi}^{(c)}_{\text{freq}} := k^{(c)}_{\text{sem}} / N$ is the unbiased sample-mean estimator of $\mu_c$ with no prior smoothing. 
%
The Bayesian proxy in \eqnref{eq:bayesian_smooth_estimation} admits the convex form
\begin{equation}
    \hat{\pi}^{(c)}_{\text{teacher}} = \frac{N}{N+\alpha}\,\hat{\pi}^{(c)}_{\text{freq}} + \frac{\alpha}{N+\alpha}\,\bar{\pi}^{(c)}_\theta.
    \label{eq:bayesian_convex_form}
\end{equation}
%
All expectations are conditional on the student trajectory $\hat{y}$; only teacher rollouts are random.


\subsection{Gradient Stability of \ours}
\label{subsec:gradient_stability}
Both standard OPD and a hypothetical \ours with empirical frequentist estimator produce gradient signals unstable enough to derail training.
%
Standard OPD's reverse-KL objective explodes when teacher mass vanishes on student-sampled tokens~\citep{fu2026revisiting}; \ours with empirical estimation collapses when teacher rollouts fail to match the student's chunk. 
%
Both failures concentrate on the same place where the teacher disagrees with the student, which are precisely the places that carry the most useful learning signal. 
%
A correct design must close both failure modes simultaneously. 
%
The theorem in this subsection establishes that \ours does so through two distinct mechanisms operating on two distinct components of the design.
%

Standard OPD's reverse-KL objective in \eqnref{eq:opd_loss} contains per-token terms of the form $\log\bigl(\pi_\theta(v) / \pi^*_{\text{teacher}}(v)\bigr)$, which diverge whenever the teacher assigns near-zero probability mass to a token the student samples. 
%
Recent analyses~\citep{fu2026revisiting,li2026rethinking,luo2026demystifying} document this as a real failure mode of token-level OPD. 
%
The chunk-level loss in \eqnref{eq:omniopd_loss} was constructed to rule out this behavior by design. 
%
The teacher estimator enters as a bounded multiplier in $[0,1]$ on the student's log-likelihood, not as a denominator or inside a log, so the per-chunk gradient is controlled by the student's score function alone---independent of what the estimator returns or how badly the teacher disagrees with $y_c$.
%

This loss change does not, however, prevent every gradient failure. 
%
Under the most direct logit-free estimator---the empirical sample mean $\hat{\pi}^{(c)}_{\text{freq}} = k^{(c)}_{\text{sem}}/N$---the estimator collapses to \emph{exactly} zero whenever none of the $N$ teacher rollouts achieves semantic match with the student chunk. 
%
A zero multiplier in \eqnref{eq:omniopd_loss} zeros out the per-chunk gradient entirely, leaving the student with no learning signal at exactly the chunks where correction is most valuable. 
%
The Bayesian prior in \eqnref{eq:bayesian_smooth_estimation} closes this gap. 
%
Because $\bar{\pi}^{(c)}_\theta > 0$ contributes a strictly positive term to the estimator at every chunk, the multiplier stays bounded away from zero regardless of the rollout outcome.
%
Essentially, the student's base-model confidence acts as a fallback signal when the teacher disagrees on every rollout.
%

The Bayesian prior does more than prevent collapse. 
%
The convex combination $\hat{\pi}^{(c)}_{\text{teacher}} = \tfrac{N}{N+\alpha}\hat{\pi}^{(c)}_{\text{freq}} + \tfrac{\alpha}{N+\alpha}\bar{\pi}^{(c)}_\theta$ introduces a bias-variance tradeoff parameterized by the prior strength $\alpha$: larger $\alpha$ reduces estimator noise but pulls the estimate further from the true teacher, while smaller $\alpha$ inherits the empirical frequentist estimator's variance under small $N$. 
%
Neither extreme is optimal---the empirical frequentist limit ($\alpha \to 0$) is dominated by sampling noise, while the pure base-prior limit ($\alpha \to \infty$) ignores teacher rollouts entirely. 
%
Since $\hat{\pi}^{(c)}_{\text{teacher}}$ enters \eqnref{eq:omniopd_loss} as a multiplier on the per-chunk gradient, the estimator's variance carries directly into the gradient's variance, which makes this tradeoff a matter of gradient stability rather than statistical accuracy alone.
%

\begin{theorem}[Gradient stability of \ours]
\label{thm:gradient_stability}
Under the chunk-level loss in \eqnref{eq:omniopd_loss} and the Bayesian path estimator from \eqnref{eq:bayesian_smooth_estimation}, the following three properties hold.
%

\textbf{(a) Loss design eliminates the gradient explosion of standard OPD.} 
For every realization of teacher rollouts and every estimator value $\hat{\pi}^{(c)}_{\text{teacher}} \in [0,1]$, the per-chunk gradient is bounded by the student's score function:
\begin{equation}
\begin{split}
    \Bigl\| \hat{\pi}^{(c)}_{\text{teacher}} &\sum_{t \in c} \nabla_\theta \log \pi_\theta(y_t \mid x, y_{<t}) \Bigr\| \\
    &\leq \sum_{t \in c}\bigl\| \nabla_\theta \log \pi_\theta(y_t \mid x, y_{<t}) \bigr\|.
\end{split}
    \label{eq:bounded_chunk_gradient}
\end{equation}
%
In contrast, the per-token gradient under the reverse-KL objective in \eqnref{eq:opd_loss} is unbounded as $\pi^*_{\text{teacher}}(v \mid x, y_{<t}) \to 0$ for any sampled token $v$.
%

\textbf{(b) Bayesian prior eliminates the supervision collapse of the empirical estimator.} 
For every realization, including the worst case $k^{(c)}_{\text{sem}} = 0$,
%
\begin{equation}
    \hat{\pi}^{(c)}_{\text{teacher}} \;\geq\; \frac{\alpha \, \bar{\pi}^{(c)}_\theta}{N + \alpha} \;>\; 0,
    \label{eq:lower_bound_estimator}
\end{equation}
%
so the per-chunk gradient remains strictly nonzero. 
%
The empirical frequentist estimator $\hat{\pi}^{(c)}_{\text{freq}}$ does not satisfy this property: under $k^{(c)}_{\text{sem}} = 0$, the chunk's gradient contribution vanishes entirely.
%

\textbf{(c) Bias-variance characterization.} 
The Bayesian estimator's mean squared error admits the closed-form bias-variance decomposition
%
\begin{equation}
\begin{split}
    \mathrm{MSE}\bigl(\hat{\pi}^{(c)}_{\text{teacher}}\bigr) &= \underbrace{\frac{N \sigma^2_\phi}{(N+\alpha)^2}}_{\text{variance}} \\
    &\quad + \underbrace{\frac{\alpha^2 \bigl(\bar{\pi}^{(c)}_\theta - \mu_c\bigr)^2}{(N+\alpha)^2}}_{\text{squared bias}},
\end{split}
    \label{eq:mse_decomposition}
\end{equation}
%
where $\sigma^2_\phi := \mathrm{Var}_{y' \sim \pi^*_{\text{teacher}}}[\phi(y_c, y')] \leq 1/4$ by Popoviciu's inequality~\citep{popoviciu1965certaines}. 
%
The two terms admit a finite optimum $\alpha^*$, and the variance strictly contracts relative to the empirical frequentist baseline: $\mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{teacher}}\bigr) = \bigl(\tfrac{N}{N+\alpha}\bigr)^2 \mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{freq}}\bigr) < \mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{freq}}\bigr)$.
\end{theorem}
%

\begin{proof}
\emph{(a)} Since $\hat{\pi}^{(c)}_{\text{teacher}} \in [0,1]$ as a convex combination of $\hat{\pi}^{(c)}_{\text{freq}} \in [0,1]$ and $\bar{\pi}^{(c)}_\theta \in [0,1]$, the triangle inequality together with $\hat{\pi}^{(c)}_{\text{teacher}} \leq 1$ gives \eqnref{eq:bounded_chunk_gradient}. 
%
For the reverse-KL contrast, the gradient
%
\begin{align*}
\nabla_\theta D_{\mathrm{KL}}&\bigl(\pi_\theta \,\|\, \pi^*_{\text{teacher}}\bigr) \\
&= \sum_v \nabla_\theta \pi_\theta(v) \,\log\frac{\pi_\theta(v)}{\pi^*_{\text{teacher}}(v)}
\end{align*}
%
contains terms whose magnitude diverges as $\pi^*_{\text{teacher}}(v) \to 0$ for any token $v$ with $\pi_\theta(v) > 0$.

\emph{(b)} From the convex form $\hat{\pi}^{(c)}_{\text{teacher}} = (k^{(c)}_{\text{sem}} + \alpha \bar{\pi}^{(c)}_\theta)/(N+\alpha)$, the setup assumption $\bar{\pi}^{(c)}_\theta > 0$, and the non-negativity of the semantic match count $k^{(c)}_{\text{sem}} \geq 0$,
%
\begin{equation*}
    \hat{\pi}^{(c)}_{\text{teacher}} \;=\; \frac{k^{(c)}_{\text{sem}} + \alpha \bar{\pi}^{(c)}_\theta}{N+\alpha} \;\geq\; \frac{\alpha \bar{\pi}^{(c)}_\theta}{N+\alpha} \;>\; 0.
\end{equation*}
%
The empirical frequentist estimator $\hat{\pi}^{(c)}_{\text{freq}} = k^{(c)}_{\text{sem}}/N$ admits no such lower bound: when $k^{(c)}_{\text{sem}} = 0$, $\hat{\pi}^{(c)}_{\text{freq}} = 0$.

\emph{(c)} Conditional on the student trajectory $\hat{y}$, the prior $\bar{\pi}^{(c)}_\theta$ is fixed and only the empirical frequentist estimator is random. 
%
Since the rollouts are i.i.d.\ with $\phi(y_c, y^{(i)}_{\text{teacher}}) \in [0,1]$,
%
\begin{align*}
    \mathbb{E}\bigl[\hat{\pi}^{(c)}_{\text{freq}}\bigr] &= \mu_c, \\
    \mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{freq}}\bigr) &= \frac{\sigma^2_\phi}{N},
\end{align*}
where $\sigma^2_\phi \leq \tfrac{1}{4}$ by Popoviciu's inequality~\citep{popoviciu1965certaines}.
%
Applying the convex form from \eqnref{eq:bayesian_convex_form}, the bias and variance of the Bayesian estimator decompose as
%
\begin{align*}
    \mathrm{Bias}\bigl(\hat{\pi}^{(c)}_{\text{teacher}}\bigr) &= \frac{N}{N+\alpha}\mu_c + \frac{\alpha}{N+\alpha}\bar{\pi}^{(c)}_\theta - \mu_c \\
    &= \frac{\alpha\bigl(\bar{\pi}^{(c)}_\theta - \mu_c\bigr)}{N+\alpha}, \\
    \mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{teacher}}\bigr) &= \Bigl(\frac{N}{N+\alpha}\Bigr)^2 \mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{freq}}\bigr) \\
    &= \frac{N \sigma^2_\phi}{(N+\alpha)^2}.
\end{align*}
%
Summing squared bias and variance yields \eqnref{eq:mse_decomposition}. The variance contraction is immediate: $(N/(N+\alpha))^2 < 1$ for all $\alpha > 0$.
\end{proof}


\subsection{Rollout Sufficiency of \ours}
\label{subsec:rollout_sufficiency}
\ours's efficiency advantage over standard OPD rests entirely on the rollout budget per chunk being small. 
%
The per-sample cost analysis in \appref{app:cost_analysis} shows that the default configuration ($M=10$, $N=10$, $C=50$) runs at 1.75$\times$ SFT cost and the sparser variant ($M=5$, $N=10$, $C=50$) runs at 0.88$\times$, but this favorable cost profile collapses entirely if accurate estimation requires $N$ on the order of hundreds or thousands. 
%
The theorem in this subsection establishes that $N=10$ is principled rather than budget-constrained, by characterizing how the estimator's accuracy improves with the rollout budget $N$ and predicting the diminishing returns observed in \tabref{tab:cost_analysis}.
%

The remaining question is whether a sparse configuration such as $N = 10$ gives a usable signal. 
%
Two effects work in \ours's favor. 
%
First, the empirical estimator $\hat{\pi}^{(c)}_{\text{freq}}$ is a sample mean over $N$ i.i.d.\ rollouts bounded in $[0,1]$, so by Hoeffding's inequality~\citep{hoeffding1963probability} its deviation from $\mu_c$ shrinks at sub-Gaussian rate in $N$. 
%
Second, the Bayesian shrinkage in \eqnref{eq:bayesian_smooth_estimation} tightens this further by a factor of $N/(N+\alpha) < 1$. 
%
Since $\hat{\pi}^{(c)}_{\text{teacher}}$ enters \eqnref{eq:omniopd_loss} as a multiplier on the per-chunk gradient, both the estimator's accuracy and the gradient noise improve at rate $\mathcal{O}(1/N)$. 
%
The marginal benefit of doubling $N$ therefore halves with each doubling, predicting a sweet spot beyond which additional rollouts purchase variance reduction that the optimizer cannot exploit.
%

\begin{theorem}[Concentration of the chunk-level estimator]
\label{thm:concentration}
For any $\varepsilon > 0$, the Bayesian chunk-level estimator concentrates around its shrunken target $\tilde{\mu}_c := \tfrac{N}{N+\alpha}\mu_c + \tfrac{\alpha}{N+\alpha}\bar{\pi}^{(c)}_\theta$ with sub-Gaussian rate
%
\begin{equation}
\begin{split}
    \Pr\!\left(\big|\hat{\pi}^{(c)}_{\text{teacher}} - \tilde{\mu}_c\big| \geq \varepsilon\right) \\
    \leq 2\exp\!\left(-\frac{2(N+\alpha)^2 \varepsilon^2}{N}\right).
\end{split}
    \label{eq:concentration_bound}
\end{equation}
%
Consequently, the estimator-induced contribution to the per-chunk gradient variance is bounded by
%
\begin{equation}
\begin{split}
    \mathrm{Var}\!&\left(\hat{\pi}^{(c)}_{\text{teacher}}\sum_{t \in c} \nabla_\theta \log \pi_\theta(y_t \mid x, y_{<t}) \,\Big|\, \hat{y}\right) \\
    &\leq \frac{N}{4(N+\alpha)^2}\Big\|\sum_{t \in c}\nabla_\theta \log \pi_\theta(y_t \mid x, y_{<t})\Big\|^2,
\end{split}
    \label{eq:concentration_variance}
\end{equation}
%
shrinking at rate $\mathcal{O}(1/N)$ in the rollout budget.
\end{theorem}
%

\begin{proof}
Conditional on the student trajectory $\hat{y}$, decompose 
$\hat{\pi}^{(c)}_{\text{teacher}} - \tilde{\mu}_c = \tfrac{N}{N+\alpha}\bigl(\hat{\pi}^{(c)}_{\text{freq}} - \mu_c\bigr)$. 
%
Applying Hoeffding's inequality~\citep{hoeffding1963probability} to $\hat{\pi}^{(c)}_{\text{freq}}$ as an average of $N$ i.i.d.\ samples in $[0,1]$,
%
\begin{equation*}
    \Pr\!\left(\big|\hat{\pi}^{(c)}_{\text{freq}} - \mu_c\big| \geq \delta\right) \leq 2\exp(-2N\delta^2),
\end{equation*}
%
and substituting $\delta = \tfrac{N+\alpha}{N}\varepsilon$ yields \eqnref{eq:concentration_bound}.
%
For the variance bound, the score sum $\sum_{t \in c} \nabla_\theta \log \pi_\theta(y_t \mid x, y_{<t})$ is deterministic conditional on $\hat{y}$, so the gradient variance factorizes as $\mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{teacher}}\bigr) \cdot \bigl\|\sum_{t \in c} \nabla_\theta \log \pi_\theta(y_t \mid x, y_{<t})\bigr\|^2$. 
%
Substituting $\mathrm{Var}\bigl(\hat{\pi}^{(c)}_{\text{teacher}}\bigr) \leq N / 4(N+\alpha)^2$ from \theoremref{thm:gradient_stability}(c) gives \eqnref{eq:concentration_variance}.
\end{proof}
%


\subsection{Un-audited Token Stability of \ours}
\label{subsec:un_audited_stability}
\ours audits only $M \cdot C$ tokens per trajectory and leaves the remaining $T - M \cdot C$ tokens un-audited. 
%
This sparsity is the design feature that makes \ours efficient---one teacher query per chunk rather than per token. 
%
However, without any constraint on the un-audited region, the student can exploit the sparse audited supervision in ways that degrade the trajectory globally, including collapsing entropy on un-audited tokens to shorten trajectories and reduce penalty mass, generating incoherent connective text between audited chunks, or shifting probability mass on un-audited tokens to satisfy gradients from the audited chunks at the cost of long-horizon fluency.
%

The KL anchor against the frozen base policy $\pi_{\text{ref}}$ closes these failure modes by constraining the un-audited region directly. 
%
At each un-audited token, Pinsker's inequality~\citep{pinsker1964information} bounds the total-variation distance between $\pi_{\text{ref}}$ and $\pi_\theta$ by the per-token KL, so reducing per-token KL through the anchor term directly bounds the per-token drift. 
%
At the aggregate level, $\theta_{\text{ref}}$ is always a feasible point of the objective at which the anchor's per-token KL terms vanish, so the optimality of $\theta^*$ forces an aggregate constraint. 
%
The total KL summed over un-audited tokens at $\theta^*$ cannot exceed the chunk-level loss improvement $\mathcal{L}_{\text{chunk}}(\theta_{\text{ref}}) - \mathcal{L}_{\text{chunk}}(\theta^*)$ divided by $\beta$.
%
Beyond a regularization weight, $\beta$ therefore has a concrete operational meaning, i.e., $\beta^{-1}$ is the exchange rate at which \ours converts chunk-level loss improvement into permitted un-audited drift.
%
\theoremref{theorem:trust_region} below makes both bounds precise---the pointwise total-variation control from Pinsker's inequality, and the aggregate KL budget that scales inversely with $\beta$.
%

\begin{theorem}[Trust-region bound on un-audited tokens]
\label{theorem:trust_region}
At any iterate $\theta$ and for every un-audited position $t \in \mathcal{U}$,
%
\begin{equation}
\begin{split}
    D_{\mathrm{TV}}\!&\bigl(\pi_{\text{ref}}(\cdot \mid x, y_{<t}) \,\|\, \pi_\theta(\cdot \mid x, y_{<t})\bigr) \\
    &\leq \sqrt{\tfrac{1}{2}D_{\mathrm{KL}}\!\bigl(\pi_{\text{ref}}(\cdot \mid x, y_{<t}) \,\|\, \pi_\theta(\cdot \mid x, y_{<t})\bigr)}.
\end{split}
    \label{eq:tv_pinsker}
\end{equation}
%
Furthermore, any minimizer $\theta^* = \arg\min_\theta \mathcal{L}_{\ours}(\theta)$ of \eqnref{eq:omniopd_loss} satisfies the aggregate budget
%
\begin{equation}
\begin{split}
    \sum_{t \in \mathcal{U}} D_{\mathrm{KL}}\!&\bigl(\pi_{\text{ref}}(\cdot \mid x, y_{<t}) \,\|\, \pi_{\theta^*}(\cdot \mid x, y_{<t})\bigr) \\
    &\leq \frac{1}{\beta}\Bigl[\mathcal{L}_{\text{chunk}}(\theta_{\text{ref}}) - \mathcal{L}_{\text{chunk}}(\theta^*)\Bigr].
\end{split}
    \label{eq:kl_budget}
\end{equation}
%
As $\beta \to \infty$, the aggregate un-audited drift vanishes and $\pi_{\theta^*} \to \pi_{\text{ref}}$ on $\mathcal{U}$.
\end{theorem}
%

\begin{proof}
The pointwise total-variation bound in \eqnref{eq:tv_pinsker} is Pinsker's inequality applied at each $t \in \mathcal{U}$. 
%
For the aggregate budget in \eqnref{eq:kl_budget}, evaluate $\mathcal{L}_{\ours}$ at the feasible point $\theta_{\text{ref}}$, where the KL anchor term vanishes by construction:
%
\begin{align*}
    \mathcal{L}_{\text{chunk}}(\theta^*) \;+\; &\beta \sum_{t \in \mathcal{U}} D_{\mathrm{KL}}\bigl(\pi_{\text{ref}} \,\|\, \pi_{\theta^*}\bigr) \\
    &\leq \mathcal{L}_{\ours}(\theta^*) \\
    &\leq \mathcal{L}_{\ours}(\theta_{\text{ref}}) \;=\; \mathcal{L}_{\text{chunk}}(\theta_{\text{ref}}),
\end{align*}
%
using optimality of $\theta^*$ and the vanishing of the KL term at $\theta_{\text{ref}}$. 
%
Rearranging yields the stated budget. 
%
The limiting statement $\pi_{\theta^*} \to \pi_{\text{ref}}$ as $\beta \to \infty$ follows because the right-hand side is bounded above by a constant independent of $\beta$, so the aggregate KL must tend to zero.
%
\end{proof}
%


\subsection{Tokenizer- and Style-Invariant Supervision}
\label{subsec:stylistic_invariance}
In the logit-free setting that \ours addresses, the natural token-level alternative is sequence-level distillation~\citep{kim2016sequence}---sample $N$ teacher rollouts and apply token-level cross-entropy on each rollout as if it were a ground-truth sequence. 
%
The resulting supervision forces the student to match the teacher's surface-form choices token by token, conflating semantic content with stylistic and formatting decisions. 
%
Standard OPD, although not directly comparable in the logit-free setting, exhibits a structurally analogous property at the distributional level---its reverse-KL objective in \eqnref{eq:opd_loss} contains terms $\log \pi^*_{\text{teacher}}(v \mid x, y_{<t})$ summed against every vocabulary token $v$, so the student inherits the teacher's full per-token preferences, including distinctions that are semantically irrelevant.
%

\ours's chunk-level loss decouples semantic content from surface form by routing all teacher information through the semantic similarity function $\phi$. 
%
The Bayesian estimator $\hat{\pi}^{(c)}_{\text{teacher}}$ depends on rollouts only through $k^{(c)}_{\text{sem}}$, and the loss in \eqnref{eq:omniopd_loss} depends on rollouts only through this estimator. 
%
Any invariance property $\phi$ has is therefore inherited by the chunk-level loss. 
%
\theoremref{thm:invariant_supervision} below formalizes this inheritance and contrasts it with the two token-level alternatives above.
%

\begin{theorem}[Tokenizer and stylistic invariance of the chunk-level loss]
\label{thm:invariant_supervision}
Let $\sim_\phi$ denote the equivalence relation on token sequences induced by $\phi$: $y \sim_\phi y'$ iff $\phi(z, y) = \phi(z, y')$ for every $z$. 
%
For any two sets of teacher rollouts $\{y^{(i)}_{\text{teacher}}\}_{i=1}^N$ and $\{y'^{(i)}_{\text{teacher}}\}_{i=1}^N$ that are $\sim_\phi$-equivalent (i.e., $y^{(i)}_{\text{teacher}} \sim_\phi y'^{(i)}_{\text{teacher}}$ for every $i$), the chunk-level Bayesian estimator and the chunk-level loss in \eqnref{eq:omniopd_loss} are invariant:
%
\begin{equation}
\begin{split}
    \hat{\pi}^{(c)}_{\text{teacher}}\bigl(\{y^{(i)}_{\text{teacher}}\}\bigr) &= \hat{\pi}^{(c)}_{\text{teacher}}\bigl(\{y'^{(i)}_{\text{teacher}}\}\bigr), \\
    \mathcal{L}_{\text{chunk}}\bigl(\theta; \{y^{(i)}_{\text{teacher}}\}\bigr) &= \mathcal{L}_{\text{chunk}}\bigl(\theta; \{y'^{(i)}_{\text{teacher}}\}\bigr).
\end{split}
    \label{eq:invariant_supervision}
\end{equation}
%
In contrast, the sequence-level distillation loss
%
\begin{equation}
\begin{split}
    \mathcal{L}_{\text{SFT}}\bigl(\theta; \{y^{(i)}_{\text{teacher}}\}\bigr) := \\
    -\frac{1}{N} \sum_{i=1}^N \sum_{t} \log &\pi_\theta\bigl(y^{(i)}_{\text{teacher}, t} \mid x, y^{(i)}_{\text{teacher}, <t}\bigr)
\end{split}
    \label{eq:sft_rollouts_loss}
\end{equation}
%
depends on specific teacher tokens and is not invariant under $\sim_\phi$-substitution. 
%
The standard OPD loss in \eqnref{eq:opd_loss} depends on the teacher's per-token distribution $\pi^*_{\text{teacher}}$ and distinguishes $\sim_\phi$-equivalent tokens whenever the teacher assigns them different probabilities.
\end{theorem}
%

\begin{proof}
The chunk-level loss in \eqnref{eq:omniopd_loss} depends on the teacher rollouts $\{y^{(i)}_{\text{teacher}}\}$ only through the Bayesian estimator $\hat{\pi}^{(c)}_{\text{teacher}}$ from \eqnref{eq:bayesian_smooth_estimation}, which in turn depends on the rollouts only through $k^{(c)}_{\text{sem}} = \sum_i \phi(y_c, y^{(i)}_{\text{teacher}, c})$. 
%
By the definition of $\sim_\phi$, $\phi(y_c, y^{(i)}_{\text{teacher}, c}) = \phi(y_c, y'^{(i)}_{\text{teacher}, c})$ for every $i$, so $k^{(c)}_{\text{sem}}$ is invariant, $\hat{\pi}^{(c)}_{\text{teacher}}$ is invariant, and $\mathcal{L}_{\text{chunk}}$ is invariant. 
%
The non-invariance of the sequence-level distillation loss in \eqnref{eq:sft_rollouts_loss} is immediate from its definition---it contains $\log \pi_\theta(y^{(i)}_{\text{teacher}, t} \mid \cdot)$ evaluated at the specific teacher tokens, which generally differ between $\sim_\phi$-equivalent rollouts. 
%
For standard OPD, \eqnref{eq:opd_loss} sums $\pi_\theta(v \mid \cdot) \log \pi^*_{\text{teacher}}(v \mid \cdot)$ over the entire vocabulary, so the loss is sensitive to any per-token distinction in $\pi^*_{\text{teacher}}$, including those between $\sim_\phi$-equivalent tokens.
\end{proof}
%

\begin{remark}[Three invariance classes]
\label{rem:invariance_classes}
The choice of $\phi$ determines which surface-level variations the chunk-level loss treats as equivalent, yielding three practically important invariance properties.
%

\textbf{Tokenizer invariance.} 
If $\phi$ operates on detokenized text---for instance, an embedding-based semantic similarity over decoded strings---then the chunk loss is invariant to the teacher's tokenizer. 
%
Teachers with different vocabularies and tokenization schemes yield the same supervision signal up to $\phi$.
%

\textbf{Paraphrase invariance.} 
If $\phi$ captures chunk-level semantic equivalence, teacher rollouts that paraphrase the same content yield identical chunk loss. 
%
The student is not penalized for choosing a different surface realization of the same semantic content.
%

\textbf{Stylistic invariance.} 
If $\phi$ is insensitive to register, formatting, or hedging conventions, teacher rollouts that differ only in stylistic dimensions yield identical chunk loss.
%

The empirical generalization of \ours across the Qwen3-32B~\citep{yang2025qwen3} and Gemini-2.5-flash~\citep{comanici2025gemini} teachers in later \secref{sec:result_analysis}---two model families with different tokenizers, training data, and stylistic preferences---is consistent with these invariance properties.
%
\end{remark}

==> sections/5_experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experiment Setup}
\label{subsec:setup}

\paragraph{Models.}
We employ Qwen3-4B and Qwen3-1.7B~\citep{yang2025qwen3} as the student models for policy optimization. 
%
To demonstrate the generalizability of our framework across both open-weight and closed-source models, we utilize a diverse suite of frontier models as oracles. 
%
Specifically, our teacher ensemble comprises the open-weights Qwen3-32B and Qwen3-30B-A3B-Instruct \citep{yang2025qwen3}, alongside the proprietary, API-gated Gemini-2.5-Flash \citep{huang2025gemini} and Claude-4.5-Haiku models \citep{Claude-4}.

\paragraph{Datasets and Evaluation.} We utilize the DAPO-Math-17K dataset \citep{yu2025dapo} to train mathematical reasoning capabilities, benchmarking downstream performance on AIME-2024 \citep{li2024numinamath}, AIME-2025, AMC23 \citep{li2024numinamath}, MATH-500 \citep{hendrycks2021measuring}, and OlympiadBench \citep{he2024olympiadbench}. 
%
Following the established setup of prior work \citep{liang2025beyond}, our code generation models are trained on the PRIME-RL compilation \citep{cui2025process}, including APPS, CodeContests, TACO, and Codeforces, and evaluated against 100 randomly sampled validation instances per dataset category.
%
To ensure statistical robustness, model performance across all domains is quantified using the Pass@1 metric, with reported results averaged over 16 independent sampling trials.


\paragraph{Baselines.} To evaluate the efficacy of our proposed framework, we benchmark against established paradigms tailored to teacher accessibility. 
%
Our primary reinforcement learning baseline is GRPO. When utilizing closed-source teachers, we compare against standard SFT, which represents the traditional off-policy limitation for proprietary models. 
%
For open-weight teachers, where full log-probabilities are accessible, we benchmark against a comprehensive two-stage pipeline consisting of SFT followed by standard white-box OPD.

\paragraph{Implementation Details.}
For our \ours framework, the default hyperparameters are configured to $M=10$ intermediate process chunks, a chunk length of $C=50$ tokens, and $N=10$ teacher MC rollouts per fork. The Reference KL anchoring penalty is weighted at $\beta = 0.1$, and we employ Edit Distance \citep{navarro2001guided} as the default semantic similarity metric ($\phi$). We systematically explore the impact of the chunk count, chunk length, rollout budget, KL weight, and choice of semantic measurer in our sensitivity analysis (\secref{sec:ablation_studies}). Other details are shown in \appref{app:imple}


\paragraph{Empirical Verification of the Bayesian Estimator.}
Before evaluating downstream reasoning performance, we validate the accuracy of our proxy estimation method using an open-weights oracle (Qwen3-32B). As detailed in Appendix \ref{sec:appendix_empirical_verification}, our analysis confirms that the Bayesian estimator strictly dominates the frequentist baseline across all evaluated semantic metrics and sample sizes. By systematically reducing Mean Squared Error (MSE) and improving Pearson correlation with the true probability density, these results empirically validate the variance reduction guarantees established in Theorem \ref{thm:gradient_stability}. Furthermore, the analysis reveals a critical trade-off between absolute magnitude accuracy (best captured by unigram metrics like ROUGE-1) and rank correlation (maximized by Edit Distance). We systematically compare the downstream impact of this specific trade-off in our sensitivity analysis (\secref{sec:ablation_studies}).


\begin{table*}[t]
\centering
\caption{Main results on mathematical reasoning benchmarks. Best results for each setup are in \textbf{bold}.}
\label{tab:main_results_math}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccc}
\toprule
\textbf{Student Model} & \textbf{Teacher Model} & \textbf{Method} & \textbf{MATH-500} & \textbf{AIME-24} & \textbf{AIME-25} & \textbf{AMC-23} & \textbf{OlympiadBench} & \textbf{Average} \\
\midrule
\multicolumn{9}{c}{\textit{Reference Models (Zero-Shot / Base Inference)}} \\
\midrule
- & Qwen3-32B & Base & 73.60 & 75.42 & 68.33 & 87.81 & 52.93 & 71.62 \\
- & Qwen3-30B-A3B-Inst. & Base & 69.81 & 61.04 & 44.79 & 78.59 & 56.38 & 62.12 \\
- & Claude-4.5-haiku & Base & 89.95 & 55.20 & 34.79 & 87.50 & 62.69 & 66.03 \\
- & Gemini-2.5-flash & Base & 86.83 & 74.79 & 65.20 & 93.13 & 61.86 & 76.36 \\
\midrule
\multicolumn{9}{c}{\textit{Student: Qwen3-1.7B}} \\
\midrule
Qwen3-1.7B & - & Base & 60.26 & 48.54 & 37.50 & 75.16 & 37.90 & 51.87 \\
Qwen3-1.7B & - & GRPO & 80.35 & 47.50 & 44.45 & 84.06 & 55.67 & 62.41 \\
\cmidrule{1-9}
\multirow{3}{*}{Qwen3-1.7B} & \multirow{3}{*}{Qwen3-32B} & SFT & 79.91 & 35.42 & 30.20 & 71.09 & 52.19 & 53.76 \\
 & & OPD & \textbf{84.82} & \textbf{48.95} & \textbf{37.58} & 79.06 & 58.08 & \textbf{61.70} \\
 & & \ours & 84.61 & 47.08 & 33.33 & \textbf{79.68} & \textbf{58.64} & 60.67 \\
\midrule
\multicolumn{9}{c}{\textit{Student: Qwen3-4B}} \\
\midrule
Qwen3-4B & - & Base & 61.55 & 50.83 & 41.88 & 75.47 & 40.32 & 54.01 \\
Qwen3-4B & - & GRPO & 73.75 & 68.62 & 60.70 & 95.93 & 52.19 & 70.24 \\
\cmidrule{1-9}
\multirow{3}{*}{Qwen3-4B} & \multirow{3}{*}{Qwen3-32B} & SFT & 68.46 & 60.83 & 58.95 & 83.59 & 47.19 & 63.80 \\
 & & OPD & 67.50 & 61.45 & 60.25 & 82.65 & 48.96 & 64.16 \\
 & & \ours & \textbf{72.60} & \textbf{68.67} & \textbf{60.42} & \textbf{93.44} & \textbf{50.27} & \textbf{69.08} \\
\cmidrule{1-9}
\multirow{3}{*}{Qwen3-4B} & \multirow{3}{*}{Qwen3-30B-A3B-Inst.} & SFT & 66.77 & 34.58 & 31.04 & 70.16 & 46.29 & 49.77 \\
 & & OPD & 69.78 & 48.54 & 36.87 & 75.78 & 50.14 & 56.22 \\
 & & \ours & \textbf{74.98} & \textbf{75.00} & \textbf{62.92} & \textbf{92.65} & \textbf{56.05} & \textbf{72.32} \\
\cmidrule{1-9}
\multirow{2}{*}{Qwen3-4B} & \multirow{2}{*}{Claude-4.5-haiku} & SFT & 80.56 & 60.83 & 53.33 & 85.16 & 57.71 & 67.52 \\
 & & \ours & \textbf{81.28} & \textbf{72.08} & \textbf{65.63} & \textbf{91.25} & \textbf{64.35} & \textbf{74.92} \\
\cmidrule{1-9}
\multirow{2}{*}{Qwen3-4B} & \multirow{2}{*}{Gemini-2.5-flash} & SFT & 80.10 & 71.25 & 63.13 & 90.44 & 62.61 & 73.51 \\
 & & \ours & \textbf{83.30} & \textbf{73.13} & \textbf{64.37} & \textbf{92.96} & \textbf{64.58} & \textbf{75.67} \\
\bottomrule
\end{tabular}%
}
\end{table*}

\subsection{Main Results}
\label{sec:result_analysis}

\paragraph{Significant Improvements over SFT Baselines.}
We present the main empirical results for mathematical reasoning and competitive programming in \tabref{tab:main_results_math} and \tabref{tab:main_results_coding} in \appref{app:programming}. 
%
Across both domains, \ours achieves substantial performance gains over the standard SFT. 
%
For instance, applying \ours to the Qwen3-4B student yields an average mathematical accuracy of 69.08\% using the open-weight Qwen3-32B as the teacher. 
%
This represents a +15.07\% absolute improvement over base model inference (54.01\%) and a robust +5.28\% gain over the SFT baseline (63.80\%). 
%
Crucially, this performance scales remarkably when integrating frontier black-box models. 
%
When distilling from Claude-4.5-haiku, \ours achieves 74.92\%, decisively outperforming its corresponding SFT baseline (67.52\%) by +7.40\%. 
%
% Similarly, using Gemini-2.5-flash as the teacher yields 75.67\%, directly surpassing the Gemini-derived SFT baseline (73.51\%) by +2.16\%. 
%
These results validate that learning from the student's own actively generated reasoning trajectories, and systematically correcting its specific bottlenecks, provides a fundamentally richer learning signal than merely imitating offline demonstrations.

\paragraph{Surpassing White-Box OPD via Bayesian Estimation.} 
Beyond outperforming offline baselines, \ours frequently exceeds standard OPD, despite OPD possessing full white-box access to the teacher's exact logits. 
%
In the Qwen3-4B to Qwen3-32B setup, \ours achieves an average of 69.08\% compared to OPD's 64.16\%. 
%
We hypothesize this advantage stems from our chunk-level Bayesian formulation acting as a statistical regularizer. Standard OPD enforces strict token-by-token imitation, heavily penalizing the student for valid alternative phrasing. 
%
By verifying multi-step chunks via semantic similarity, \ours grants the student local structural flexibility. 
%
It extracts a smoother, more robust gradient signal that focuses on reaching correct reasoning milestones rather than matching deterministic token sequences.

\paragraph{Teacher Capacity Scaling and Comparisons to GRPO.} 
The impact of teacher capacity on distillation efficacy becomes particularly evident when comparing our method against reinforcement learning paradigms (GRPO). 
%
When paired with a relatively bounded open-weight teacher (e.g., Qwen3-32B teaching Qwen3-1.7B), \ours (60.67\%) slightly trails the self-improving GRPO baseline (62.41\%). 
%
This suggests that when the teacher's capability margin over the student is small, the self-exploration of GRPO under a rule-based environment reward remains highly competitive. 
%
However, as we scale the teacher to frontier models, \ours rapidly unlocks performance ceilings that GRPO cannot reach. 
%
When the Qwen3-4B student is trained via \ours using Claude-4.5-haiku (74.92\%) or Gemini-2.5-flash (75.67\%), it decisively surpasses the 4B GRPO baseline (70.24\%). 
%
This confirms that \ours effectively bridges the capability divide between open and closed-source models, allowing smaller student networks to harness the vast reasoning capacity of frontier models to surpass standard RLHF limits.

\paragraph{Training Dynamics.}
To understand the optimization stability and learning progression of \ours, we track the training dynamics of the Qwen3-4B student under both open-weights (Qwen3-32B) and frontier black-box (Gemini-2.5-flash) teachers. As detailed in Appendix \ref{sec:appendix_training_dynamics}, the chunk-level on-policy loss exhibits rapid, monotonic convergence, empirically validating the gradient stability guarantees of our Bayesian smoothing mechanism (Theorem \ref{thm:gradient_stability}). Simultaneously, the KL divergence between the active policy and the frozen base model safely plateaus, perfectly mirroring the un-audited token bounds established in Theorem \ref{theorem:trust_region}. This stable optimization translates directly into continuous progression on downstream evaluations, driving rapid accuracy gains on the challenging AIME-2025 dataset and proving the efficacy of our peak-entropy chunk scheduling.

==> sections/6_ablations.tex <==
\section{Ablation Studies and Analysis}

\begin{table}[t]
\centering
\caption{Ablation study of \ours components on mathematical reasoning.}
\label{tab:ablation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
\textbf{Variant} & \textbf{MATH} & \textbf{AIME-24} & \textbf{AIME-25} & \textbf{AMC-23} & \textbf{Olympiad} & \textbf{Avg} \\
\midrule
\ours (Full) & 72.60 & 68.67 & \textbf{60.42} & \textbf{93.44} & \textbf{50.27} & \textbf{69.08} \\
\midrule
w/o Entropy Selection & 70.35 & \textbf{70.42} & 58.54 & 92.69 & 50.26 & 68.45 \\
w/o Bayesian Smoothing & \textbf{72.95} & 70.00 & 58.29 & 91.87 & 50.04 & 68.63 \\
w/o KL Anchoring & 9.27 & 8.13 & 6.25 & 12.03 & 5.71 & 8.28 \\
\bottomrule
\end{tabular}%
}
\end{table}

\subsection{Ablation Studies}
\label{sec:ablation_studies}

To isolate the empirical contribution of each core mechanism in the \ours framework, we conduct a systematic ablation study using the Qwen3-4B student and Qwen3-32B teacher setup. 
%
The results, presented in \tabref{tab:ablation}, strongly validate the theoretical properties established in \appref{sec:theoretical_analysis}. 

The most dramatic impact is observed when removing the base-model KL penalty ($\beta = 0$). 
%
Without this regularization, the student's average performance catastrophically collapses from 69.08\% to 8.28\%. 
%
This corroborates Theorem \ref{theorem:trust_region}: because our framework only audits $M$ discrete chunks, creating vast unsupervised gaps in the generated trajectory, the absence of a KL constraint allows the policy to rapidly degenerate. 
%
The student exploits the sparse verification signals, ultimately losing its foundational linguistic fluency and structural reasoning coherence. 

Beyond the necessity of the trust region, we also validate the impact of our statistical and scheduling mechanisms. 
%
Replacing our Bayesian proxy with standard frequentist estimation degrades the overall average accuracy from 69.08\% to 68.63\%. While the model maintains baseline functionality, the lack of Bayesian smoothing exposes the optimization process to the severe estimation error inherent in limited black-box sampling (Theorem \ref{thm:gradient_stability}). 
%
Finally, we substitute our peak-entropy anchored selection with a naive uniform sampling strategy, which further reduces the overall average to 68.45\%.
%
Anchoring the verification chunks strictly at points of maximum predictive entropy ensures the teacher's corrective signal is concentrated exactly where the student policy faces critical, uncertain decision boundaries. 
%
To provide concrete intuition for how this peak-entropy scheduling, we also provide detailed case studies in \appref{sec:appendix_case_studies}.

\begin{table}[t]
\centering
\caption{Sensitivity analysis of \ours hyperparameters: verification budget ($M$), Monte Carlo rollouts ($N$), and chunk size ($C$).}
\label{tab:sensitivity_hyperparams}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
\toprule
$M$ & $N$ & $C$ & \textbf{MATH} & \textbf{AIME-24} & \textbf{AIME-25} & \textbf{AMC-23} & \textbf{Olympiad} & \textbf{Avg} \\
\midrule
10 & 10 & 50 & 72.60 & 68.67 & 60.42 & 93.44 & 50.27 & 69.08 \\
\midrule
5 & 10 & 50 & 72.76 & 69.58 & 55.63 & 93.44 & 50.48 & 68.38 \\
10 & 10 & 25 & 52.73 & 10.42 & 4.79 & 32.19 & 22.26 & 24.48 \\
\midrule
10 & 20 & 50 & 73.35 & 68.54 & 61.04 & 93.13 & 51.81 & 69.57 \\
20 & 10 & 50 & 75.01 & 70.63 & \textbf{62.71} & 90.94 & 55.50 & 70.96 \\
10 & 10 & 100 & \textbf{75.94} & \textbf{72.29} & 62.50 & \textbf{93.59} & 53.58 & \textbf{71.58} \\
\midrule
10 & 20 & 100 & 75.00 & 72.08 & 61.88 & 93.13 & \textbf{55.72} & 71.56 \\
\bottomrule
\end{tabular}%
}
\end{table}

\subsection{Sensitivity Analysis}
\label{sec:sensitivity_analysis}

To understand the robustness of \ours, we analyze its sensitivity to its core hyperparameters: the chunk number ($M$), the Monte Carlo rollout count ($N$), the chunk size ($C$), the Bayesian prior ($\alpha$), and the semantic measurement function ($\phi$). 
%
The results, utilizing the Qwen3-4B student and Qwen3-32B teacher, are detailed in \tabref{tab:sensitivity_hyperparams} and \tabref{tab:sensitivity_semantic_metric}.

\paragraph{Sensitivity to Verification Hyperparameters.}
Our analysis reveals distinct scaling dynamics across the three core hyperparameters governing the verification budget. 
%
The framework is most sensitive to the verification chunk size ($C$); expanding to $C=100$ yields the highest overall average performance (71.58\%) by providing richer structural context for the Bayesian proxy, whereas halving the baseline to $C=25$ causes a catastrophic drop to 24.48\%. 
%
This confirms that overly narrow windows make the semantic similarity metric excessively noisy, penalizing phrasing differences rather than verifying logical deduction. 
%
In contrast, scaling Monte Carlo rollouts ($N$) exhibits rapidly diminishing returns. Increasing from $N=10$ to $N=20$ provides negligible improvements (+0.49\% at $C=50$, and fractional losses at $C=100$), demonstrating that $N=10$ safely occupies the Pareto frontier for capturing semantic variance without unjustifiably doubling API query costs. 
%
Finally, \ours proves remarkably resilient regarding the total number of audited chunks ($M$). 
%
While increasing to $M=20$ boosts the average to 70.96\% via denser supervision, aggressively reducing the budget to $M=5$ results in only a minimal performance dip to 68.38\%. 
%
This robustness empirically validates our peak-entropy anchored scheduling (\secref{subsubsec:speculative_verification})—by strictly targeting high-uncertainty decision boundaries, the corrective gradient signals remain potent enough to preserve final reasoning capabilities even under massive cost reductions (see \appref{app:cost_analysis} for a detailed scalability analysis).

\begin{table}[t]
\centering
\caption{Sensitivity analysis of the semantic measurement function ($\phi$). We compare normalized Edit Distance against ROUGE-1 unigram overlap across different student-teacher pairings.}
\label{tab:sensitivity_semantic_metric}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllcccccc}
\toprule
\textbf{Student Model} & \textbf{Teacher Model} & \textbf{Metric ($\phi$)} & \textbf{MATH} & \textbf{AIME-24} & \textbf{AIME-25} & \textbf{AMC-23} & \textbf{Olympiad} & \textbf{Avg} \\
\midrule
\multirow{2}{*}{Qwen3-1.7B} & \multirow{2}{*}{Qwen3-32B} & Edit Distance & 84.61 & 47.08 & 33.33 & 79.68 & \textbf{58.64} & 60.67 \\
 & & ROUGE-1 & \textbf{86.30} & \textbf{48.13} & \textbf{36.46} & \textbf{85.31} & 58.16 & \textbf{62.87} \\
\midrule
\multirow{2}{*}{Qwen3-4B} & \multirow{2}{*}{Qwen3-32B} & Edit Distance & \textbf{72.60} & 68.67 & 60.42 & \textbf{93.44} & 50.27 & 69.08 \\
 & & ROUGE-1 & 70.36 & \textbf{72.71} & \textbf{61.04} & 92.18 & \textbf{50.52} & \textbf{69.36} \\
\midrule
\multirow{2}{*}{Qwen3-4B} & \multirow{2}{*}{Qwen3-30B} & Edit Distance & \textbf{74.98} & \textbf{75.00} & \textbf{62.92} & 92.65 & \textbf{56.05} & \textbf{72.32} \\
 & & ROUGE-1 & 74.78 & 71.67 & 61.88 & \textbf{93.75} & 55.72 & 71.56 \\
\bottomrule
\end{tabular}%
}
\end{table}


\paragraph{Impact of the Bayesian Prior ($\alpha$).}
The parameter $\alpha$ controls the strength of the base-model prior during our Bayesian smoothing step. 
%
As illustrated in \figref{fig:alpha_sensitivity}, \ours exhibits a distinct performance peak at $\alpha=1.0$. 
%
Deviating from this optimal balance in either direction results in performance degradation, illustrating the bias-variance tradeoff inherent in discrete sampling. 
%
When the prior is too weak ($\alpha=0.1$), the average accuracy drops to 67.52\%, the framework overfits to the severe statistical variance and zero-probability traps of the $N=10$ discrete Monte Carlo rollouts. 
%
Conversely, applying an overly aggressive prior ($\alpha \geq 4.0$) causes a steep performance collapse. 
%
In this high-$\alpha$ regime, the trust-region penalty becomes too restrictive, forcing the student to stubbornly anchor to its own sub-optimal base policy and effectively blocking it from learning the teacher's advanced reasoning trajectories.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/alpha_sensitivity.pdf}
    \caption{Sensitivity of \ours to the Bayesian prior ($\alpha$). $\alpha=1.0$ achieves the optimal balance between smoothing Monte Carlo variance and policy updates.}
    \label{fig:alpha_sensitivity}
\end{figure}


\paragraph{Robustness to Semantic Measurement Functions.}
While \ours is highly robust to the choice of semantic metric $\phi$ (\tabref{tab:sensitivity_semantic_metric}), the optimal selection depends heavily on the student-teacher capacity gap. 
%
For heavily constrained students (1.7B) learning from large base models (32B), ROUGE-1 significantly outperforms Edit Distance (+2.20\% average).
%
Because smaller models struggle to perfectly mimic verbose teacher structures, Edit Distance is overly punitive; ROUGE-1 instead provides crucial linguistic flexibility. As student capacity scales to 4B, this gap narrows (+0.28\% average). 
%
Conversely, when distilling a highly aligned instruction-tuned teacher into a 4B student, Edit Distance yields a slight edge (+0.76\% average). 
%
This suggests ROUGE-1 is ideal for bridging extreme capacity mismatches, while Edit Distance excels at enforcing the strict structural mimicking required for aligned reasoning.

==> sections/7_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we introduced \ours, a logit-free, chunk-level OPD framework that addresses both the white-box access requirement of standard OPD and the brittleness of its token-level supervision signal. By unifying peak-entropy chunk scheduling, Bayesian-smoothed speculative verification, and base-model KL anchoring, our approach efficiently extracts robust, variance-reduced gradient signals from teacher models while mathematically bounding policy degeneration. Extensive evaluations demonstrate that \ours not only matches the performance of standard OPD but also scales seamlessly to proprietary models. Ultimately, \ours bridges the closed-source capability divide, empowering smaller open-weight models to harness the reasoning capacity of frontier models and comprehensively surpass the traditional limits of offline fine-tuning and self-exploratory reinforcement learning.


\section{Limitations}
\label{sec:limitations}

While \ours significantly stabilizes on-policy distillation, its effectiveness remains inherently bounded by the capabilities of the chosen teacher and the precision of the semantic measurement function ($\phi$). As demonstrated in our sensitivity analysis, the optimal choice of $\phi$ fluctuates depending on the student-teacher capacity gap and the structural alignment of the models. Consequently, if the framework is applied to highly subjective domains where reasoning validity cannot be reliably captured by automated structural or unigram metrics, the Bayesian proxy may struggle to isolate an accurate supervisory signal. Furthermore, because the peak-entropy scheduling heavily anchors the student to the teacher's trajectory distributions at critical junctions, the method remains susceptible to inheriting systemic biases or compounding hallucinatory reasoning steps if the frontier oracle exhibits underlying flaws.

Additionally, although our chunk-level formulation drastically reduces the query volume by a factor of $\mathcal{O}(T/C)$ compared to token-level continuous oversight, the speculative verification process still imposes a non-trivial computational overhead during the training phase. Generating $N$ Monte Carlo rollouts per audited chunk requires high-throughput inference infrastructure, which can become a bottleneck when scaling the framework to ultra-long context windows, such as multi-file repository-level code generation or extensive legal analysis. While our $M=5$ budget configuration proves highly resilient, future work must explore dynamic rollout sizing or more aggressive pruning strategies to further compress the computational footprint without sacrificing the mathematical integrity of the Bayesian estimator.


\section{Ethical Considerations}
We utilized GPT-based models \citep{openai2023gpt4} solely for language polishing and proofreading.
%
This work studies training methods for knowledge distillation using public benchmark environments and does not introduce new datasets containing personal or sensitive information.
%
\ours{} relies on teacher judgments, so biases or unsafe preferences in the teacher model may be propagated to the student.
%
Practical deployment should therefore include appropriate action validation, safety constraints, logging, and human oversight.



